Contextually Plausible and Diverse 3D Human Motion Prediction

We tackle the task of diverse 3D human motion prediction, that is, forecasting multiple plausible future 3D poses given a sequence of observed 3D poses. In this context, a popular approach consists of using a Conditional Variational Autoencoder (CVAE). However, existing approaches that do so either fail to capture the diversity in human motion, or generate diverse but semantically implausible continuations of the observed motion. In this paper, we address both of these problems by developing a new variational framework that accounts for both diversity and context of the generated future motion. To this end, and in contrast to existing approaches, we condition the sampling of the latent variable that acts as source of diversity on the representation of the past observation, thus encouraging it to carry relevant information. Our experiments demonstrate that our approach yields motions not only of higher quality while retaining diversity, but also that preserve the contextual information contained in the observed 3D pose sequence.

==> figures/cq_plot.tex <==
\pgfplotsset{width=0.49\textwidth, height=0.35\textwidth, compat=1.3, legend columns=1, legend style={at={(0.23,0.9)},anchor=north}, grid style={dashed,gray}}  
% \usetikzlibrary{plotmarks}
% \usetikzlibrary{backgrounds}
\begin{tikzpicture}
\scriptsize
\begin{axis}[
    legend cell align={left},
	ylabel={\footnotesize Context},
	xlabel={\footnotesize Quality},
	ytick={0,.1,.2, .3, .4, 0.5},
	xtick={0, .5, .1,.15, .2,.25, .3,.35, .4, .45, 0.5},
	legend image post style={scale=0.0},
	grid=both
]

% \addplot [mark=*, mark size=2pt, blue]
% 	coordinates {(0.48, 0.53)}
% 	node[above] at (axis cs:0.42, 0.50) {\tiny Ours};
\node[] at (axis cs: 0.38,0.06) {\textbf{\textit{Note: Marker radius indicates Diversity.}}};
	
\addplot [mark=*, mark size=7.04pt, olive]
	coordinates {(0.42, 0.37)}
	node[above] at (axis cs:0.36, 0.35) {\footnotesize Mix\&Match}; 
	\addlegendentry{\small Mix-and-Match~\cite{aliakbarian2019MixAndMatch}}
	
\addplot [mark=*, mark size=9.4pt, red]
	coordinates {(0.44, 0.29)}
	node[above] at (axis cs:0.44, 0.21) {\footnotesize DLow}; \addlegendentry{\small DLow~\cite{yuan2020dlow}}

\addplot [mark=*, mark size=0.96pt, teal]
	coordinates {(0.47, 0.35)}
	node[above] at (axis cs:0.48, 0.35) {\footnotesize HP-GAN}; \addlegendentry{\small HP-GAN~\cite{yuan2020dlow}}
	
\addplot [mark=*, mark size=3.4pt, orange]
	coordinates {(0.13, 0.08)}
	node[above] at (axis cs:0.185, 0.06) {\footnotesize Pose-Knows}; \addlegendentry{\small Pose-Knows~\cite{walker2017pose}}
	
\addplot [mark=*, mark size=0.52pt, blue]
	coordinates {(0.45, 0.42)}
	node[above] at (axis cs:0.45, 0.42) {\footnotesize MT-VAE}; \addlegendentry{\small MT-VAE~\cite{yan2018mt}}
	
\addplot [mark=*, mark size=6.24pt, black]
	coordinates {(0.48, 0.54)}
	node[above] at (axis cs:0.40, 0.52) {\footnotesize LCP-VAE (Ours)}; \addlegendentry{\small LCP-VAE (Ours)}
	

\end{axis}
\end{tikzpicture}

==> latex/figures/cq_plot.tex <==
\pgfplotsset{width=0.49\textwidth, height=0.35\textwidth, compat=1.3, legend columns=1, legend style={at={(0.23,0.9)},anchor=north}, grid style={dashed,gray}}  
% \usetikzlibrary{plotmarks}
% \usetikzlibrary{backgrounds}
\begin{tikzpicture}
\scriptsize
\begin{axis}[
    legend cell align={left},
	ylabel={\footnotesize Context},
	xlabel={\footnotesize Quality},
	ytick={0,.1,.2, .3, .4, 0.5},
	xtick={0, .5, .1,.15, .2,.25, .3,.35, .4, .45, 0.5},
	legend image post style={scale=0.0},
	grid=both
]

% \addplot [mark=*, mark size=2pt, blue]
% 	coordinates {(0.48, 0.53)}
% 	node[above] at (axis cs:0.42, 0.50) {\tiny Ours};
\node[] at (axis cs: 0.38,0.06) {\textbf{\textit{Note: Marker radius indicates Diversity.}}};
	
\addplot [mark=*, mark size=7.04pt, olive]
	coordinates {(0.42, 0.37)}
	node[above] at (axis cs:0.36, 0.35) {\footnotesize Mix\&Match}; 
	\addlegendentry{\small Mix-and-Match~\cite{aliakbarian2019MixAndMatch}}
	
\addplot [mark=*, mark size=9.4pt, red]
	coordinates {(0.44, 0.29)}
	node[above] at (axis cs:0.44, 0.21) {\footnotesize DLow}; \addlegendentry{\small DLow~\cite{yuan2020dlow}}

\addplot [mark=*, mark size=0.96pt, teal]
	coordinates {(0.47, 0.35)}
	node[above] at (axis cs:0.48, 0.35) {\footnotesize HP-GAN}; \addlegendentry{\small HP-GAN~\cite{yuan2020dlow}}
	
\addplot [mark=*, mark size=3.4pt, orange]
	coordinates {(0.13, 0.08)}
	node[above] at (axis cs:0.185, 0.06) {\footnotesize Pose-Knows}; \addlegendentry{\small Pose-Knows~\cite{walker2017pose}}
	
\addplot [mark=*, mark size=0.52pt, blue]
	coordinates {(0.45, 0.42)}
	node[above] at (axis cs:0.45, 0.42) {\footnotesize MT-VAE}; \addlegendentry{\small MT-VAE~\cite{yan2018mt}}
	
\addplot [mark=*, mark size=6.24pt, black]
	coordinates {(0.48, 0.54)}
	node[above] at (axis cs:0.40, 0.52) {\footnotesize LCP-VAE (Ours)}; \addlegendentry{\small LCP-VAE (Ours)}
	

\end{axis}
\end{tikzpicture}
